The Behavior and Convergence of Local Bayesian Optimization

A recent development in Bayesian optimization is the use of local optimization strategies, which can deliver strong empirical performance on high-dimensional problems compared to traditional global strategies. The "folk wisdom" in the literature is that the focus on local optimization sidesteps the curse of dimensionality; however, little is known concretely about the expected behavior or convergence of Bayesian local optimization routines. We first study the behavior of the local approach, and find that the statistics of individual local solutions of Gaussian process sample paths are surprisingly good compared to what we would expect to recover from global methods. We then present the first rigorous analysis of such a Bayesian local optimization algorithm recently proposed by M\"uller et al. (2021), and derive convergence rates in both the noisy and noiseless settings.

==> miscellaneous.tex <==

Let $GP\bb{0, k}$ be a GP defined on a compact set $\Xc \subseteq \sbb{0, 1}^d$ with zero mean and the kernel $k$.
Let $f \sim GP\bb{0, k}$.

\begin{fact}[Bounded Derivative]
Let $f$ be a function draw from the prior GP.
Then, $\frac{\partial f}{\partial x_i}$ is a function draw from the derivative GP.
Thanks to the compactness of the domain $\Xc$, the supremum of the derivative
\begin{align*}
    \sup_{\xv \in \Xc} \abs{\frac{\partial f}{\partial x_i}}
\end{align*}
is finite almost surely.\footnote{In fact, it is always finite.}
According to the Borell-TIS inequality, the following two are finite\footnote{$b_i$ is the derivative's variance, which is automatically bounded if the kernel satisfies $\sup_{\xv \in \Xc} k\bb{\xv, \xv} < \infty$.}
\begin{align*}
    & \Eb\sbb{\sup_{\xv \in \Xc} \abs{\frac{\partial f}{\partial x_i}}} < \infty, \\
    & b_i^2 = \sup_{\xv \in \Xc} \Eb\sbb{\bb{\frac{\partial f}{\partial x_i}}^2} < \infty.
\end{align*}
Furthermore, we have
\begin{align*}
    \prob{\sup_{\xv \in \Xc} \abs{\frac{\partial f}{\partial x_i}} > \Eb\sbb{\sup_{\xv \in \Xc} \abs{\frac{\partial f}{\partial x_i}}} + u} \leq \exp\bb{- \frac{u^2}{2 b_i^2}}.
\end{align*}
\end{fact}

\begin{lemma}[$\ell_\infty$-Lipschitzness of Function Draws]
Let $f$ be a function draw from the GP.
Let $L$ be the Lipschitz constant of $f$
\begin{align*}
    L = \sup_{\xv \in \Xc} \norm{\nabla f\bb{\xv}}_1.
\end{align*}
Then, we have
\begin{align*}
    \prob{L > \sum_{i=1}^{d} \Eb\sbb{\sup_{\xv \in \Xc} \abs{\frac{\partial f}{\partial x_i}}} + du} \leq d\exp\bb{- \frac{u^2}{2 b_i^2}}
\end{align*}
\end{lemma}

\begin{proof}
All we need to prove is $f$ has bounded the gradient in $\ell_1$ norm w.h.p.
\begin{align*}
    \sup_{\xv \in \Xc} \norm{\nabla f\bb{\xv}}_1 & = \sup_{\xv \in \Xc} \sum_{i = 1}^{d} \abs{\frac{\partial f}{\partial x_i}} \\
    & \leq \sum_{i = 1}^{d} \sup_{\xv \in \Xc} \abs{\frac{\partial f}{\partial x_i}}.
\end{align*}
Apply Borell-TIS inequality to the last line and use union bound.
\end{proof}

\begin{remark}
Note that the fucntions in the RKHS $\Hc$ are also Lipschitz.
Assuming bounded norm, their Lipschitz constants are also bounded.
\end{remark}



\subsection{The Discretization Argument}

\begin{lemma}
Let the domain $\Xc \subseteq \sbb{0, 1}^d$ be compact.
We discretize the domain using a grid with $\bb{\frac{1}{\epsilon}}^d$ many samples.
With high probability we have
\begin{align*}
    f\bb{\xv^*} - \max_i f\bb{\xv_i} \leq L \epsilon,
\end{align*}
where $L = \sup_{\xv \in \Xc} \norm{\nabla f\bb{\xv}}_1$ which satisfies the high probability bound in the previous lemma.
\end{lemma}

\begin{proof}
Due to discretization, we have
\begin{align*}
    \min_i \norm{\xv^* - \xv_i}_\infty \leq  \epsilon.
\end{align*}
Let $\xv_{\mathrm{near}}$ be the point closest to $\xv^*$ in infinity norm.
We have
\begin{align*}
    f\bb{\xv^*} - \max_i f\bb{\xv_i} & \leq f\bb{\xv^*} - f\bb{\xv_{\mathrm{near}}} \\
    & \leq L \norm{\xv^* - \xv_{\mathrm{near}}}_\infty \\
    & \leq L \epsilon.
\end{align*}
\end{proof}

Next, we want to show that there exists a subset on the grid that approximates $\max_i f\bb{\xv_i}$ well, so that we do not actually need $\bb{\frac{1}{\epsilon}}^d$ many samples.

Here are a few existing results on bounding the maximum of (possibly correlated) Gaussian random variables \parencite{hartigan2014bounding, ross2010computing}. 
\textcite[Lemma 3.3]{grunewalder2010regret} mentioned a result
\begin{align*}
    \Eb\sbb{\max_{1 \leq i \leq n} X_i} = \sigma \sqrt{2 \log n},
\end{align*}
regardless whether $X_i$'s are independent or not.

\begin{lemma}
\label{lma:convergence-constant-error}
Assume that $f$ is $\beta$-smooth.
Suppose the gradient oracle $\gv_t$ satisfies
$\norm{\nabla f\bb{\xv_t} - \gv_t} \leq c \norm{\nabla f\bb{\xv_t}}$
for all $t$ and for some constant $0 < c < 1$.
Then, the $T$ iterations of the following update
\begin{align*}
    \xv_{t + 1} = \xv_t - \eta_t \gv_t
\end{align*}
with step size $\eta_t = \frac{1}{\beta}$ gives
\begin{align*}
    \min_{1 \leq t \leq T} \norm{\nabla f\bb{\xv_t}}^2 \leq \frac{2 \beta \bb{f\bb{\xv_1} - f^*}}{\bb{1 - c} T}.
\end{align*}
\end{lemma}

\begin{proof}
By $\beta$-smoothness, we have
\begin{align*}
    f\bb{\xv_{t + 1}} \leq f\bb{\xv_t} + \nabla f\bb{\xv_t}^\top \bb{\xv_{t + 1} - \xv_t} + \frac12 \beta \norm{\xv_{t + 1} - \xv_t}^2.
\end{align*}
Using the assumption on the gradient oracle, we have
\begin{align*}
    f\bb{\xv_{t + 1}} \leq f\bb{\xv_t} - \frac{1 - c}{2 \beta} \norm{\nabla f\bb{\xv_t}}^2.
\end{align*}
Telescoping sum finishes the proof.
\end{proof}

It is well known that the posterior mean function is the minimum norm interpolant in $\Hc$.
Namely, $\mu_{\Dc}$ is the unique minimum of the following problem \parencite{wendland2004scattered}
\begin{align}
    & \mini_{f \in \Hc} \quad \norm{f}_\Hc \\
    & \sbjto ~ f\bb{\xv_i} = y_i, \quad i = 1, 2, \cdots, n.
\end{align}
The gradient estimate is $\nabla \mu_{\Dc}\bb{\zv}$.
Our goal in this section is to characterize the worst-case estimation error
\begin{align*}
    \sup_{f \in \Hc} \norm{\nabla f\bb{\zv} - \nabla \mu_{\Dc}\bb{\zv}}
\end{align*}
where the location $\zv$ is fixed, the dataset is denoted as $\Dc = \cbb{\xv_i}_{i = 1}^{n}$ and the labels are $y_i = f\bb{\xv_i}$.

Write $\mu_{\Dc}$ in an alternative form as a weighted sum of functions, which will turn out to be useful:
\begin{align*}
    \mu_\Dc\bb{\cdot} & = \yv^\top \Kv^{-1} k\bb{\Xv, \cdot} \\
    & = \sum_{i = 1}^{n} f\bb{\xv_i} u_i\bb{\cdot},
\end{align*}
where each $u_i\bb{\cdot}: \Rb^d \to \Rb$ is defined as
\begin{align*}
\bb{u_1\bb{\cdot}, u_2\bb{\cdot}, \cdots, u_n\bb{\cdot}}^\top = \Kv^{-1} k\bb{\Xv, \cdot}
\end{align*}

